Evidence of Fragmenting Dust Particles from Near-Simultaneous Optical and Near-IR Photometry and Polarimetry of Comet 73P/Schwassmann-Wachmann 3

We report imaging polarimetry of segments B and C of the Jupiter-family Comet 73P/Schwassmann-Wachmann 3 in the I and H bandpasses at solar phase angles of approximately 35 and 85deg. The level of polarization was typical for active comets, but larger than expected for a Jupiter-family comet. The polarimetric color was slightly red (dP/dL = +1.2 +/- 0.4) at a phase angle of ~ 35deg and either neutral or slightly blue at a phase angle of ~ 85deg. Observations during the closest approach from 2006 May 11-13 achieved a resolution of 35 km at the nucleus. Both segments clearly depart from a 1/rho surface brightness for the first 50 - 200 km from the nucleus. Simulations of radiation driven dust dynamics can reproduce some of the observed coma morphology, but only with a wide distribution of initial dust velocities (at least a factor of 10) for a given grain radius. Grain aggregate breakup and fragmentation are able to reproduce the observed profile perpendicular to the Sun-Comet axis, but fit the observations less well along this axis (into the tail). The required fragmentation is significant, with a reduction in the mean grain aggregate size by about a factor of 10. A combination of the two processes could possibly explain the surface brightness profile of the comet.

==> tab1.tex <==
\begin{deluxetable}{ccccc}
\tablenum{1}
\tablewidth{0pt}
\tablecaption{Observing Log}
\tablehead{
\colhead{Date (2006)} & \colhead{UT (Hr)} & \colhead{Telescope} & \colhead{Instrument} & \colhead{Filter}
}
\startdata

April 18 & 3:35 & MLOF & OPTIPOL & $I$ \\
April 18 & 9:30 & Perkins & Mimir & $H$ \\
April 19 & 5:41 & MLOF & OPTIPOL & $I$ \\
April 19 & 8:15 & Perkins & Mimir & $H$ \\
May 11 & 9:30 & MLOF & OPTIPOL & $I$ \\
May 12 & 10:08 & MLOF & OPTIPOL & $I$ \\
May 12 & 13:32 & IRTF & NSFCAM2 & $H$ \\
May 13 & 8:26 & MLOF & OPTIPOL & $I$ \\
May 13 & 13:26 & IRTF & NSFCAM2 & $H$ \\

\enddata
\end{deluxetable}

==> tab2.tex <==
\begin{deluxetable}{cccccccc}
\tablenum{2}
\tablewidth{0pt}
\tablecaption{Aperture Polarimetry $(3\arcsec)$}
\tablehead{
\colhead{Date (2006)} & \colhead{UT (Hr)} & \colhead{Segment} & Phase Angle & \colhead{Filter} & \colhead{P(\%)} &\colhead{$\epsilon P(\%)$} & \colhead{$\Delta$ (AU)} }
\startdata

April 18 & 3:35 & C & 35.8 & $I$ & 6.0 & 0.2 & 0.227 \\
April 18 & 9:03 & C & 36.0 & $H$ & 7.0 & 0.3 & 0.225 \\
April 19 & 5:41 & B & 35.1 & $I$ & 5.5 & 0.2 & 0.233 \\
April 19 & 8:15 & B & 35.6 & $H$ & 6.5 & 0.3 & 0.232 \\
May 11 & 9:30 & B & 78.2 & $I$ & 22.7 & 0.2 & 0.071 \\
May 12 & 10:08 & C & 87.3 & $I$ & 24.4 & 0.2 & 0.079 \\
May 12 & 13:32 & C & 87.9 & $H$ & 23.5 & 0.3 & 0.079 \\
May 12 & 8:26 & B & 82.9 & $I$ & 23.8 & 0.2 & 0.069\\
May 13 & 13:26 & B & 88.6 & $H$ & 24.5 & 0.3 & 0.067 \\

\enddata
\end{deluxetable}
